Autoregressive regularized score-based diffusion models for multi-scenarios fluid flow prediction

Building on recent advances in scientific machine learning and generative modeling for computational fluid dynamics, we propose a conditional score-based diffusion model designed for multi-scenarios fluid flow prediction. Our model integrates an energy constraint rooted in the statistical properties of turbulent flows, improving prediction quality with minimal training, while enabling efficient sampling at low cost. The method features a simple and general architecture that requires no problem-specific design, supports plug-and-play enhancements, and enables fast and flexible solution generation. It also demonstrates an efficient conditioning mechanism that simplifies training across different scenarios without demanding a redesign of existing models. We further explore various stochastic differential equation formulations to demonstrate how thoughtful design choices enhance performance. We validate the proposed methodology through extensive experiments on complex fluid dynamics datasets encompassing a variety of flow regimes and configurations. Results demonstrate that our model consistently achieves stable, robust, and physically faithful predictions, even under challenging turbulent conditions. With properly tuned parameters, it achieves accurate results across multiple scenarios while preserving key physical and statistical properties. We present a comprehensive analysis of stochastic differential equation impact and discuss our approach across diverse fluid mechanics tasks.

==> body/2_template.tex <==
%% Use \section commands to start a section
\section{Example Section}
\label{sec1}
%% Labels are used to cross-reference an item using \ref command.

Section text. See Subsection \ref{subsec1}.

%% Use \subsection commands to start a subsection.
\subsection{Example Subsection}
\label{subsec1}

Subsection text.

%% Use \subsubsection, \paragraph, \subparagraph commands to 
%% start 3rd, 4th and 5th level sections.
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Document_Structure#Sectioning_commands

\subsubsection{Mathematics}
%% Inline mathematics is tagged between $ symbols.
This is an example for the symbol $\alpha$ tagged as inline mathematics.

%% Displayed equations can be tagged using various environments. 
%% Single line equations can be tagged using the equation environment.
\begin{equation}
f(x) = (x+a)(x+b)
\end{equation}

%% Unnumbered equations are tagged using starred versions of the environment.
%% amsmath package needs to be loaded for the starred version of equation environment.
\begin{equation*}
f(x) = (x+a)(x+b)
\end{equation*}

%% align or eqnarray environments can be used for multi line equations.
%% & is used to mark alignment points in equations.
%% \\ is used to end a row in a multiline equation.
\begin{align}
 f(x) &= (x+a)(x+b) \\
      &= x^2 + (a+b)x + ab
\end{align}

\begin{eqnarray}
 f(x) &=& (x+a)(x+b) \nonumber\\ %% If equation numbering is not needed for a row use \nonumber.
      &=& x^2 + (a+b)x + ab
\end{eqnarray}

%% Unnumbered versions of align and eqnarray
\begin{align*}
 f(x) &= (x+a)(x+b) \\
      &= x^2 + (a+b)x + ab
\end{align*}

\begin{eqnarray*}
 f(x)&=& (x+a)(x+b) \\
     &=& x^2 + (a+b)x + ab
\end{eqnarray*}

%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Mathematics
%% https://en.wikibooks.org/wiki/LaTeX/Advanced_Mathematics

%% Use a table environment to create tables.
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Tables
\begin{table}[t]%% placement specifier
%% Use tabular environment to tag the tabular data.
%% https://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular_environment
\centering%% For centre alignment of tabular.
\begin{tabular}{l c r}%% Table column specifiers
%% Tabular cells are separated by &
  1 & 2 & 3 \\ %% A tabular row ends with \\
  4 & 5 & 6 \\
  7 & 8 & 9 \\
\end{tabular}
%% Use \caption command for table caption and label.
\caption{Table Caption}\label{fig1}
\end{table}


%% Use figure environment to create figures
%% Refer following link for more details.
%% https://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions
\begin{figure}[t]%% placement specifier
%% Use \includegraphics command to insert graphic files. Place graphics files in 
%% working directory.
\centering%% For centre alignment of image.
\includegraphics{example-image-a}
%% Use \caption command for figure caption and label.
\caption{Figure Caption}\label{fig1}
%% https://en.wikibooks.org/wiki/LaTeX/Importing_Graphics#Importing_external_graphics
\end{figure}


%% The Appendices part is started with the command \appendix;
%% appendix sections are then done as normal sections
\appendix
\section{Example Appendix Section}
\label{app1}

Appendix text.

%% For citations use: 
%%       \cite{<label>} ==> [1]

%%
Example citation, See \cite{lamport94}.

%% If you have bib database file and want bibtex to generate the
%% bibitems, please use
%%
%%  \bibliographystyle{elsarticle-num} 
%%  \bibliography{<your bibdatabase>}

%% else use the following coding to input the bibitems directly in the
%% TeX file.

%% Refer following link for more details about bibliography and citations.
%% https://en.wikibooks.org/wiki/LaTeX/Bibliography_Management


==> body/6_Results/effects_of_PC.tex <==
\section{Influence of predictor-corrector approach}

SDE formulation means PC approach for free. 
Take best of all and re-sample.

Since we have access to the governing equations and a heuristic solution, we propose a PC inspired technique but for the physical time, \emph{e.g.}, a correction of the model's full state prediction over $n_{\text{GD}}$ steps. For that, the following residuals are computed:
\begin{equation}
    \begin{cases}
    \mathcal{R}_{1} = \frac{
    \rho(\bft{r},\tau+\mathrm{d}\tau) - \rho(\bft{r},\tau)}{\mathrm{d}\tau} + 
    \bdiv{_{\bft{r}}} \parenthesis{
    \rho(\bft{r}, \tau)\bft{u}(\bft{r}, \tau)} \,, \\
    \mathcal{R}_{2}=\frac{
    \rho(\bft{r},\tau+\mathrm{d}\tau) \bft{u}(\bft{r},\tau+\mathrm{d}\tau)
    - \rho(\bft{r},\tau) \bft{u}(\bft{r},\tau)}{\mathrm{d}\tau} + 
    \bdiv{_{\bft{r}}} \parenthesis{
    \rho(\bft{r}, \tau)\bft{u}(\bft{r}, \tau) \otimes \bft{u}(\bft{r}, \tau) + P(\bft{r}, \tau)\bft{I}} \,, \\
    \mathcal{R}_{3} = \frac{
    \Energy(\bft{r},\tau+\mathrm{d}\tau) - \Energy(\bft{r},\tau)}{\mathrm{d}\tau} + 
    \bnabla_\rv \cdot \left((\Energy(\bft{r},\tau) + \Pres(\bft{r},\tau))\uv(\bft{r},\tau) \right) +\frac{\Energy(\bft{r},\tau+\mathrm{d}\tau)}{\tau_{\text{cool}}} \,,
    \end{cases}
\end{equation}
keeping flux (divergence computation) as “past” states. It be optimized with through a global loss function (see \ref{algo:PINNsampling}):
\begin{equation}
    \mathcal{L}_{\text{GD}}=
    \lambda_{1}*\left\Vert \mathcal{R}_{1} \right\Vert_{2}^{2} +
    \lambda_{2}*\left\Vert \mathcal{R}_{2} \right\Vert_{2}^{2} + 
    \lambda_{3}*\left\Vert \mathcal{R}_{3} \right\Vert_{2}^{2} \,,
\end{equation}
where $\lambda_1$, $\lambda_2$ and $\lambda_3$ are scalars chosen such that each residual have an almost equal weight.

\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\caption{\hspace{-.2em}: PC sampling (VP SDE) \cite{SMSDE}}
\begin{algorithmic}[1]


\State $\mathrm{d}t = 1/N$
\State $\bx_{N}^{\tau} \sim \mathcal{N}\left( \bft{0}, \bft{I} \right)$

\Statex \colorbox{blue!10}{\parbox{\dimexpr\linewidth-2\fboxsep}{\textbf{Predictor (Euler–Maruyama solver)}}}

\For{$i = N-1$ \textbf{to} $0$}

    \State $\bft{\epsilon } \sim \mathcal{N}\left( \bft{0}, \bft{I} \right)$
    \State $\bx_{i}^{\tau} = \bx_{i+1}^{\tau} - \tilde{\bmu}(i+1) \mathrm{d}t + \bsigma(i+1) \sqrt{\mathrm{d}t} \, \bft{\epsilon}$

    \Statex \colorbox{orange!20}{\parbox{\dimexpr\linewidth-2\fboxsep}{\textbf{Corrector (Langevin steps)}}}
    
    \For{$j = 1$ \textbf{to} $n_{\text{corr}}$}

        \State $\bz \sim \mathcal{N}\left(\bft{0}, \bft{I}\right)$
        \State $\delta \gets 2  (1-\beta_{i}) \parenthesis{r \Vert \bz \Vert_{2}/\Vert \bft{s}_{\btheta^{*}}(\bx_{i}^\tau,\bx_0^{\tau-1},i) \Vert_{2}}^{2}$
        \State $\bx_{i}^{\tau} \gets \bx_{i}^{\tau} + \delta \, \bft{s}_{\btheta^{*}}(\bx_{i}^\tau,\bx_0^{\tau-1},i) + \sqrt{2\delta} \,\bft{z}$
    \EndFor
\EndFor
\State \textbf{return} $\hat{\bx}^{\tau}_0 := \bx^{\tau}_{i=0}$


\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\caption{\hspace{-.2em}: Physics-informed sampling}\label{algo:PINNsampling}
\begin{algorithmic}[1]

\State $\bx^{0}_0 \in \IC(\bx)$

\For{$\tau = 1$ \textbf{to} $\mathcal{T}$}

    \State $\bx_{N}^{\tau} \sim \mathcal{N}\left( \bft{0}, \bft{I} \right)$
    
    \Statex \colorbox{blue!10}{\parbox{\dimexpr\linewidth-2\fboxsep}{\textbf{Predictor}}}
    
    \Statex \colorbox{orange!20}{\parbox{\dimexpr\linewidth-2\fboxsep}{\textbf{Corrector}}}
    
    \State $\hat{\bx}^{\tau}_0 := \bx^{\tau}_{i=0}$
    
    \For{$i = 1$ \textbf{to} $n_{\text{GD}}$}

    \State $\hat{\bft{u}}_{0}^{\tau} \gets \hat{\bft{u}}_{0}^{\tau} - \eta_{\bft{u}} \cdot \bnabla_{\hat{\bft{u}}} \mathcal{L}_{\text{GD}}(\hat{\bft{x}}_{0}^{\tau}, \hat{\bx}_{0}^{\tau-1})$
    
    \State $\hat{\rho}_{0}^{\tau} \gets \hat{\rho}_{0}^{\tau} - \eta_{\rho} \cdot \bnabla_{\hat{\rho}} \mathcal{L}_{\text{GD}}(\hat{\bft{x}}_{0}^{\tau}, \hat{\bx}_{0}^{\tau-1})$
    
    \State $\hat{P}_{0}^{\tau} \gets \hat{P}_{0}^{\tau} - \eta_{P} \cdot \bnabla_{\hat{P}} \mathcal{L}_{\text{GD}}(\hat{\bft{x}}_{0}^{\tau}, \hat{\bx}_{0}^{\tau-1})$

    \State $\hat{\bx}^{\tau}_0 = [\hat{\bft{u}}_{0}^{\tau}, \hat{\rho}_{0}^{\tau},\hat{P}_{0}^{\tau}]$

    \EndFor
    
\EndFor

\State \textbf{return} $\set{\hat{\mathbf{x}}^{0}_0, \hat{\mathbf{x}}^{1}_0, \dots, \hat{\mathbf{x}}^{\mathcal{T}}_0}$

\end{algorithmic}
\end{algorithm}

\end{minipage}


NB. $\set{\delta_i}_i$ are step sizes and $r$ the SNR


==> body/Z_scratch.tex <==
\section{scratch -----------------------------------------------------------------------------------------------------------------}


$\bx^{\tau-1} \,\,\ \bx^{\tau} \,\,\, \bx^{\tau+1}  \,\, \bx^{\tau+2}$
$\bx^{\tau}_{0} \sim p_{data}(\cdot)$
$\bx_{T}^{\tau} \sim \mathcal{N}\left(\bft{0},\bft{I}\right)$
$\hat{\bx}_{0}^{\tau} \sim p_{0}(\cdot \lvert \bx_{0}^{\tau-1})$
$\bx^{\tau-1} \,\,\ \bx^{\tau}_t \,\,\, \bx^{\tau+1}  \,\, \bx^{\tau+2}$
$$\times\frac{-1}{\sigma_{t}}$$
$\mathcal{L}(\btheta)$





==> body/images_scrap.tex <==
% \begin{figure}[t]
% \centering
% \begin{minipage}[]{0.41\textwidth}
%     \includegraphics[width=\linewidth]{images/scrap/turbRad_spectra.png}
% \end{minipage}
% \begin{minipage}[]{0.42\textwidth}
%     \includegraphics[width=\linewidth]{images/scrap/turbRad_variance.png}
% \end{minipage}
% \includegraphics[width=\linewidth,keepaspectratio=True]{images/scrap/turbRad_SDE_compa_time=40.png}
% \caption{legend}
% \label{fig:enter-label}
% \end{figure}
% \begin{figure}[t]
% \centering
% \begin{minipage}[]{0.41\textwidth}
%     \includegraphics[width=\linewidth]{images/scrap/turbRad_spectra.png}
% \end{minipage}
% \begin{minipage}[]{0.42\textwidth}
%     \includegraphics[width=\linewidth]{images/scrap/turbRad_variance.png}
% \end{minipage}
% \end{figure}
% \begin{figure}[t]
% \includegraphics[width=\linewidth,keepaspectratio=True]{images/scrap/turbRad_SDE_compa_time=40.png}
% \caption{legend}
% \label{fig:enter-label}
% \end{figure}
